Penalty-based Numerical Representation of Rigid Body Interactions with Applications to Simulation of Robotic Grasping

This paper presents a novel approach to numerically describe the interactions between rigid bodies, with a special focus on robotic grasping. Some of the more common approaches used to address such issues rely on satisfaction of a set of strict constraints, descriptive of the expected physical reality of such interactions in practice. However, application of constraint-based methods in a numerical setting may lead to problematic configurations in which, for instance, volumes occupied by distinct bodies may overlap. Such situations lying beyond the range of admissible configurations for constraint-based methods, their occurrence typically results in non-meaningful simulation outcomes. We propose a method which acknowledges the possibility of such occurrences while demoting their occurrence. This is pursued through the use of a penalty-based approach, and draws on notions of mechanical impedance to infer apposite reaction forces. Results of numerical simulations illustrate efficacy of the proposed approach.

==> algorithm2e/doc/algorithm2e_ex01.tex <==
\SetAlgoVlined
\eIf{cond1}{
  a line\;
  a line\;
}{
  another line\;
  another line\;
}


==> algorithm2e/doc/algorithm2e_ex02.tex <==
\SetAlgoNoLine
\If{cond2}{
  second if\;
  second if\;
}


==> algorithm2e/doc/algorithm2e_ex03.tex <==
\lIf{cond3}{ another example}
\Else{
  a block\;
  a block\;
}


==> algorithm2e/doc/algorithm2e_ex04.tex <==
\lIf{cond4}{ok} \lElse{wrong}
\leIf{cond4}{ok}{wrong}


==> algorithm2e/doc/algorithm2e_ex05.tex <==
\SetAlgoVlined
\lIf{cond5}{cond5 true}
\uElseIf{cond51}{
  cond 5 false\;
  but cond51 true\;
}
\ElseIf{}{
  all is wrong\;
  \Return result52\;
}


==> algorithm2e/doc/algorithm2e_ex06.tex <==
\SetAlgoLined
\uIf{cond6}{
  cond6 is ok\;
  always ok\;
}
\uElseIf{cond62}{
  choose result62\;
  \Return result62\;
}
\Else{
  all is wrong\;
  do something else\;
}


==> algorithm2e/doc/algorithm2e_ex07.tex <==
Let's have a look at what we can do
with if-then-else and side comments\;
\eIf{if-then-else test}{
  no comment here\;
  neither in then\;
}{
  nor in else\;
}
\eIf(\tcc*[f]{then comment}){test}{
  then with a comment\;
}(\tcc*[f]{comment in else})
{
  here we are in else\;
}
\eIf(\tcc*[f]{then comment}){test}{
  again a comment in then\;
}{
  but not in else\;
}
\eIf{if-then-else test}{
  this time, no comment in then\;
}(\tcc*[f]{else comment})
{
  but one comment in else\;
}
Let's try with other if possibilities\;
\lIf(\tcc*[h]{lif comment}){test}{text}
\uIf(\tcc*[f]{uif comment}){test}{
  then text\;
}
\uElseIf(\tcc*[f]{comment}){test}{
  elseif text\;
}
\lElseIf(\tcc*[h]{comment}){test}{text}
\lElse(\tcc*[f]{comment}){text}


==> algorithm2e/doc/algorithm2e_exAlgoDisjdecomp.tex <==
\IncMargin{1em}
\begin{algorithm}
  \SetKwData{Left}{left}\SetKwData{This}{this}\SetKwData{Up}{up}
  \SetKwFunction{Union}{Union}\SetKwFunction{FindCompress}{FindCompress}
  \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}

  \Input{A bitmap $Im$ of size $w\times l$}
  \Output{A partition of the bitmap}
  \BlankLine
  \emph{special treatment of the first line}\;
  \For{$i\leftarrow 2$ \KwTo $l$}{
    \emph{special treatment of the first element of line $i$}\;
    \For{$j\leftarrow 2$ \KwTo $w$}{\label{forins}
      \Left$\leftarrow$ \FindCompress{$Im[i,j-1]$}\;
      \Up$\leftarrow$ \FindCompress{$Im[i-1,]$}\;
      \This$\leftarrow$ \FindCompress{$Im[i,j]$}\;
      \If(\tcp*[h]{O(\Left,\This)==1}){\Left compatible with \This}{\label{lt}
        \lIf{\Left $<$ \This}{\Union{\Left,\This}}
        \lElse{\Union{\This,\Left}}
      }
      \If(\tcp*[f]{O(\Up,\This)==1}){\Up compatible with \This}{\label{ut}
        \lIf{\Up $<$ \This}{\Union{\Up,\This}}
        \tcp{\This is put under \Up to keep tree as flat as possible}\label{cmt}
        \lElse{\Union{\This,\Up}}\tcp*[h]{\This linked to \Up}\label{lelse}
      }
    }
    \lForEach{element $e$ of the line $i$}{\FindCompress{p}}
  }
  \caption{disjoint decomposition}\label{algo_disjdecomp}
\end{algorithm}\DecMargin{1em}

==> algorithm2e/doc/algorithm2e_exIR.tex <==
\begin{algorithm}
\DontPrintSemicolon
\KwData{$G=(X,U)$ such that $G^{tc}$ is an order.}
\KwResult{$G'=(X,V)$ with $V\subseteq U$ such that $G'^{tc}$ is an
interval order.}
\Begin{
  $V \longleftarrow U$\;
  $S \longleftarrow \emptyset$\; 
  \For{$x\in X$}{ 
    $NbSuccInS(x) \longleftarrow 0$\;
    $NbPredInMin(x) \longleftarrow 0$\;
    $NbPredNotInMin(x) \longleftarrow |ImPred(x)|$\;
    }
  \For{$x \in X$}{
    \If{$NbPredInMin(x) = 0$ {\bf and} $NbPredNotInMin(x) = 0$}{
      $AppendToMin(x)$}
    } 
    \nl\While{$S \neq \emptyset$}{\label{InRes1}
    \nlset{REM} remove $x$ from the list of $T$ of maximal index\;\label{InResR}
    \lnl{InRes2}\While{$|S \cap  ImSucc(x)| \neq |S|$}{ 
      \For{$ y \in  S-ImSucc(x)$}{
        \{ remove from $V$ all the arcs $zy$ : \}\;
        \For{$z \in  ImPred(y) \cap  Min$}{
          remove the arc $zy$ from $V$\;
          $NbSuccInS(z) \longleftarrow NbSuccInS(z) - 1$\;
          move $z$ in $T$ to the list preceding its present list\;
          \{i.e. If $z \in T[k]$, move $z$ from $T[k]$ to 
           $T[k-1]$\}\;
          }
        $NbPredInMin(y) \longleftarrow 0$\;
        $NbPredNotInMin(y) \longleftarrow 0$\;
        $S \longleftarrow S - \{y\}$\;
        $AppendToMin(y)$\;
        }
      }
    $RemoveFromMin(x)$\;
    }
  }  
\caption{IntervalRestriction\label{IR}}
\end{algorithm}


==> algorithm2e/doc/algorithm2e_exProg.tex <==
\SetAlgoLined
\SetKwProg{Fn}{Function}{ is}{end}
\Fn{afunc(i: int) : int}{return 0\;}  

\SetKwProg{Def}{def}{:}{}
\Def{afunc(i: int)}{return 0\;}

==> algorithm2e/doc/algorithm2e_exfor.tex <==
\SetAlgoLined
\ForAll{elements of $S_1$}{
  remove an element e from $S_1$\;
  put e in the set $S_2$\;
  }
\lFor{i=1 \emph{\KwTo}max}{mark i}\;
\ForEach{$e$ in the set}{
  put $e$ in ${\cal E}$\;
  mark $e$\;
}


==> algorithm2e/doc/algorithm2e_exgeneric.tex <==
\Fn(\tcc*[h]{algorithm as a recursive function}){\FRecurs{some args}}{
  \KwData{Some input data\\these inputs can be displayed on several lines and one 
    input can be wider than line's width.}
  \KwResult{Same for output data}
  \tcc{this is a comment to tell you that we will now really start code}
  \If(\tcc*[h]{a simple if but with a comment on the same line}){this is true}{
    we do that, else nothing\;
    \tcc{we will include other if so you can see this is possible}
    \eIf{we agree that}{
      we do that\;
    }{
      else we will do a more complicated if using else if\;
      \uIf{this first condition is true}{
        we do that\;
      }
      \uElseIf{this other condition is true}{
        this is done\tcc*[r]{else if}
      }
      \Else{
        in other case, we do this\tcc*[r]{else}
      }
    }
  }
  \tcc{now loops}
  \For{\forcond}{
    a for loop\;
  }
  \While{$i<n$}{
    a while loop including a repeat--until loop\;
    \Repeat{this end condition}{
      do this things\;
    }
  }
  They are many other possibilities and customization possible that you have to
  discover by reading the documentation.
}


==> algorithm2e/doc/algorithm2e_exgeneric2.tex <==
\Fn(\tcc*[h]{algorithm as a recursive function}){\FRecurs{some args}}{
  \KwData{Some input data}
  \KwResult{Same for output data}
  \If(\tcc*[h]{a simple if but with a comment on the same line}){this is true}{
    we do that, else nothing\;
    \lIf{we agree that}{we do that}
    \Else{
      \lIf{this first condition is true}{we do that}
      \lElseIf(\tcc*[h]{else if}){this other condition is true}{this is done}
      \lElse(\tcc*[h]{else}){in other case, we do this}
    }
  }
  \lFor{\forcond}{a for loop}
  \While{$i<n$}{
    a while loop including a repeat--until loop\;
    \lRepeat(\tcc*[h]{a comment}){this end condition}{do this things}
  }
  They are many other possibilities and customization possible that you have to
  discover by reading the documentation.
}


==> algorithm2e/doc/algorithm2e_exnlsty.tex <==
\SetNlSty{texttt}{[}{]}
\SetAlgoNlRelativeSize{0}
\SetNlSkip{0em}
\nl\KwIn{input data}
\nl\KwOut{output data}
\nl\tcc{a comment line in C-style}
\nl\Repeat{\nl$e<\tau$}{
  \nl$f_n\leftarrow Y_1$\;
  \nl$f_{n+1}\leftarrow f_n\times f_{n-1}$\;
  \nl$e\leftarrow \frac{f_n}{2}$\;
}
\nl\KwRet{$e$}

==> algorithm2e/doc/algorithm2e_exrepeat.tex <==
\Repeat{this stop condition}{
  the text of the loop\;
  another line\;
  always in the loop\;
  }
\lRepeat{stop}{a one line loop}


==> algorithm2e/doc/algorithm2e_exswitch.tex <==
\Switch{the value of T}{
  \uCase{a value}{
    do this\;
    do that\;
  }
  \lCase{another value}{one line}
  \Case{last value}{
    do this\;
    break\;
  }
  \Other{
    for the other values\;
    do that\;
  }
}


==> sections/acknowledgments.tex <==
This research has received funding from the European Union’s Horizon 2020 Framework Programme for Research and Innovation under the Specific Grant Agreement No. 785907 (Human Brain Project SGA2).

==> sections/approach_approximations.tex <==
Our approach allows objects to first overlap on contact, then apply corrective forces that return them to a physically correct state. In real-life scenarios, two bodies never occupy the same space at the same time. In contrast to this, penalty-based methods must allow overlaps to occur to compute reaction efforts, which inhibits their precision in modeling rigid bodies. However, no real-life objects possess an infinite stiffness. Upon contact, objects will bend ever so slightly before returning to their original shape, thus moving their center of mass closer together. This can be mimicked by mechanical impedance, as demonstrated in \cite{jain2011controlling}. Our process mimics the brief bending and restitution in a similar manner, allowing objects to move closer together than a rigid model would allow (bending), then pushing them back to their intended distance (restitution). This effect is noticeable in grasping scenarios, where objects are bent slightly out of shape, exhibiting spring forces similar to mechanical impedance at the contact points.

==> sections/approach_contact_force_computation.tex <==
\begin{figure}
	\centering
	%\def\svgwidth{\columnwidth}
	\includesvg[width=0.9\columnwidth]{images/simple_collision_all_2.svg}
	\caption{Overlap Repulsive Force Computation(a: Sort lines to corresponding object; b: Iterate over blue line, get distance vector and force apply position, c: Calculate total force and apply position)}
	\label{fig:overlap_computation}
\end{figure}

A major aspect of physics simulation is collision detection and reaction effort computation. For penalty-based approaches such as the one we are using, this requires some form of overlap detection to determine where two or more objects are occupying the same space. As bodies do not overlap in real-life scenarios, such occurrences are penalized by applying a corrective force which push the bodies apart.

In our case, we developed a new approach to determining body overlap. First, we determine the intersecting area of two polyshapes. Should the bodies be far enough apart for no overlap to occur, the function returns an empty shape.

Once an overlap is detected, penalizing forces must be computed. The larger the area of overlap, the greater the repulsive forces that act on both objects. However, we also require a directional component that indicates the direction in which either objects should be moved, namely away from the area of overlap. 
Thirdly, once the efforts have been determined, we must also identify the force application position.

For all of these components, we require more information from the intersecting shape than just the area. Our approach iterates over the shape's outline and determines how deep the bodies penetrate at each position. The repulsive force is adjusted proportionally. The following describes the process in greater detail.
 
First, we analyze the outer lines of the overlapping shape. Each line is sorted to its corresponding object, either $\vA$ or $\vB$ (see figure \ref{fig:overlap_computation}).
Next, we iterate over the lines assigned to body $\vA$. For each line $\vlA$, we compute the normal $\vnlA$. Then, we iterate over all positions on $\vlA$ with an increment of $\vdeltaL$. At each of these positions $\vp$ along $\vlA$, we store the distance vector $\vfP$ to the closest position on all lines in $\vB$ along the normal $\vnlA$. This distance vector will be used as a component of the total repulsive force. Additionally the center $\vcP$ between $\vp$ and the aforementioned minimum distance point is also stored. $\vcP$ will be used to determine the force application position. If no line $\vlB$ can be found, the position is ignored.
%The distance vector is used as an indicator of the repulsive force that should be applied at position $\bm{c}_p$ to push both objects apart.

Once all lines of $\vA$ have been analyzed as described above, we sum up all distance vectors and center positions to
\begin{align}
	\vfEst &\triangleq \sum_{p \in \vlA}^{} \vdeltaL \vfP, \quad                             &t \geqslant 0,\\
	\vc    &\triangleq \sum_{p \in \vlA}^{} \vdeltaL \frac{||\vfP||}{||\vfEst||} \vcP, \quad &t \geqslant 0,
\end{align}
where $||\cdot||$ is the usual Euclidian norm.
$\vfEst$ will be used to estimate the repulsive forces between objects $\vA$ and $\vB$ using a PD control law (described below), and $\vc$ is the position where the force will be applied.

==> sections/introduction_VN.tex <==
\section{Introduction}\label{sec:introduction}
%
The manufacturing industry has been undergoing a radical paradigm shift over the past decade (referred to as fourth industrial revolution), brought about by the development of Information and Communications Technology (ICT). The developments involved have allowed production lines to become more agile, making it possible for instance to address specialised small product batches in a cost-effective manner (ideally, at mass production cost). A key operation involved in such production line is that of assembly. Its automation by robotic means implies the necessity for the involved robot to locate, grasp, and then place specific parts. The grasping operation is, in general, a non-trivial one. It typically involves interactions between a robotic arm with a meaningful number of Degrees of Freedom (DoFs), an object being grasped (whose physical properties of inertia might be either partially uncertain, or not straightforward to represent concisely), and an assembly onto which the grasped object must be placed or fixed. The grasping itself involves friction forces, which are notoriously challenging to model accurately. The final step involves exchange of effort between the robotic arm, the object grasped, and the assembly. Both the arm and the assembly being typically rigidly mounted, the operation involves a closed mechanical chain, which further complicates the process.

These different aspects contribute to rendering the reconfiguration process of a production line involving such assembly tasks rather complex. While it is possible to explore this design in a numerical setting, some of the dimensions involved remain challenging to faithfully, accurately model in numerical simulations. Grasping constitutes one of the more challenging aspects. A number of applications have been developed to address this problem, including \texttt{GraspIt!} and \texttt{OpenRAVE} (\cite{graspit, openrave}). They provide a number of functions, most of them accounting for static quality of considered grasps, reflecting how well a given gripper (characterised by geometry, configuration, actuation) is able to grasp a considered object. However, such static considerations fail to address the dynamic nature of usual manipulation scenarii encountered in practice, where objects are picked, moved, and placed dynamically. A number of dynamic performance metrics have been defined (\cite{roa_grasp_metrics}). Their assessment requires consideration of the dynamic nature of the considered system. Existing grasping applications commonly rely on numerical physics engines such as the Open Dynamics Engine ({ODE}) and {Bullet}. The \texttt{GraspIt!} toolbox relies on Bullet, whereas \texttt{OpenRAVE} has an interface allowing the use of either ODE and Bullet.

To simulate dynamic rigid body interactions, these engines rely on constraint-based methods (\cite{baraff1993non}). In particular, for each discrete time-step of the simulation, a set of constraints is defined, reflecting properties and situation of the considered gripper, the object being grasped, and the environment. Each constraint is intended to be descriptive of the interactions between two given rigid bodies, defining reaction forces descriptive of contacts between such bodies (including impacts, support, or reflecting exchanges of efforts in joints). From the considered constraint is inferred an appropriate effort being applied on the involved objects. For instance, hinge joint constraints define reactive forces that ensure the two considered bodies are kept in contact at the hinge position; they are left free to rotate around the specified axis, but other relative movements are entirely compensated by the constraint effort. Of particular relevance to grasping are contact constraints, which prevent objects from physically overlapping. They are implemented in a manner that is similar to the aforementioned hinge constraint. In particular, upon detection of the emergence of one such contact, a constraint enforcing non-overlap is added to the previously considered ones (see the discussion in \cite{baraff1993non}). The constraint prevents body movement in the direction of the contact point, preventing overlap. Different approaches may be used to infer appropriate efforts from the defined set of constraints, one of the most commonly encountered method formulates a Linear Complementary Problem (LPC), which may be solved using a number of different techniques (see \cite{anitescu_time_stepping_lcp_solver,lemke_lcp_solver}). Once evaluated, constraint forces are applied to concerned rigid bodies, thereby affecting their trajectory in the desired manner (see discussion in \cite{extending_ode_robots}).

Constraint-based approaches perform appropriately for a certain range of scenarii. However, a number of situations may give rise to substantial issues. For instance, rapid relative movement of objects, if simulation time steps are not carefully adjusted, may result in actual overlap between the bodies; this overlap occurring before the contact is detected and appropriate constraint forces are generated to avoid this situation. A straightforward mitigating measure to such issues consists in carefully monitoring for such abhorrences, and adjusting (that is, reducing) the simulation time-step to a degree that is commensurate with the relative velocity of the concerned objects. However, such methods add considerable complexity and offer no guarantee of success (\cite{engine_simulation}). Another situation in which such overlaps commonly occur (when working in discrete time numerical simulation) is involving closed mechanical chains. Grasping, when a gripper applies efforts on an object from different, opposing directions falls into that category. The situation is particularly prevalent when considering force-closure grasp (\cite{nguyen1988constructing}). Successfully enforcing non-overlap constraints in such situations requires particularly small simulation time steps. In the event that an overlap ends up occurring, LCP based methods typically fail, as such situations are not foreseen (\cite{baraff_analytical}).

A number of results can be found in  the literature to address such issues. A common approach involves accounting for the possibility of overlaps (which is essentially inherent to discrete-time simulation), and compute reaction forces in such a manner that, when such situations do occur, they only exist in short transient state, rapidly replaced with a steady-state situation in which contacts and interactions faithfully reflect their real-world, physical reality. The approach in [citation needed], for instance, defines a set of criteria to overcome inter-body penetrations. These result in the application of a repulsive force to overlapping objects, proportional to their relative velocity, at the point(s) of contact. The approach implies a number of additional steps to the simulation which may prove exceedingly computationally intensive, to the extent that real-time computations are in practice difficult to achieve. In addition, the defined repulsive forces can in some configurations lead to the emergence of a resonance effect, destabilizing force-closed grasps. Numerical simulation of grasping using such an approach typically requires the addition of artificial, large damping efforts diffusing excess energy (see \cite{engine_simulation}). Another approach involves the replacement of constraints with impulses to describe interactions, as in \cite{impulse_based}. The approach is able to account for overlap of rigid bodies. However, the reliance on impulses may lead to inaccuracies (see discussion in \cite{impulse_based}). A manner to directly address and account for overlaps consists in treating such instances not as anomalies, but rather as errors to be reduced (or regulated). This can be pursued by defining repulsion forces in light of these errors, in a manner that concerned objects are pushed apart, as described in \cite{drumwright_penalty_based}. Penalty-based methods offer a rapid and robust approach to address simulation scenarii in which objects intersect with each other. Their performance has been demonstrated with implementations that allow to consider thousands of objects in real-time (\cite{fast_penalty_based,drumwright_fast_penalty}). In the following, we build upon this penalty-based perspective, to develop an algorithm supporting reliable numerical simulation of robotic grasping. In particular, we ground the definition of the penalty efforts, computed from measured overlaps, in considerations of mechanical impedance (including stiffness and damping), designed to reflect the expected behavior of the considered objects in their interactions.

This paper is structured as follows. \sec{approach} provides an overview of the proposed approach, and results of illustrative numerical simulations are provided in \sec{simulations}. \sec{conclusion} concludes this paper. 

==> sections/introduction_YM.tex <==
\section{Introduction}\label{sec:introduction}
%
The manufacturing industry has been undergoing a radical paradigm shift over the past decade (referred to as fourth industrial revolution in \cite{schuh2017}), brought about by the development of Information and Communications Technology (ICT). The developments involved have allowed production lines to become more agile, making it possible for instance to address specialised small product batches in a cost-effective manner (ideally, at mass production cost). A key operation involved in a meaningful range of such production line is that of assembly. Its automation by robotic means implies the necessity for the involved robot to locate, grasp, then place specific parts. The grasping operation is, in general, a non-trivial one. It typically involves interactions between a robotic arm with a meaningful number of Degrees of Freedom (DoFs), an object being grasped (whose physical properties of inertia may be either partially uncertain, or not straightforward to represent in a concise manner), and an assembly onto which the grasped object must be placed or fixed. The grasping itself involves friction forces, which are notoriously challenging to accurately model (\cite{haessig1991}). The final step involves exchange of effort between the robotic arm, the object grasped, and the assembly. Both the arm and the assembly being typically rigidly mounted, the operation involves a closed mechanical chain, which further complicates the process.

These different aspects contribute to rendering the reconfiguration process of a production line involving such assembly tasks rather complex. While it is possible to explore this design in a numerical setting, some of the dimensions involved remain challenging to faithfully, accurately model in numerical simulations. Grasping constitutes one of the more challenging aspects. A number of applications have been developed to address this problem, including \texttt{GraspIt!} and \texttt{OpenRAVE} (\cite{graspit, openrave}). They provide a number of functions, a significant number of them accounting for static quality of considered grasps, reflecting how well a given gripper (characterised by geometry, configuration, actuation) is able to grasp a considered object. However, such static considerations fail to address the dynamic nature of usual manipulation scenarii encountered in practice, where objects are picked, moved, placed, dynamically. A number of dynamic performance metrics have been defined (\cite{roa_grasp_metrics}), their assessment requires consideration of the dynamic nature of the considered system. Existing grasping applications commonly rely on numerical physics engines such as the Open Dynamics Engine (\texttt{ODE} \cite{smith2005}) and \texttt{Bullet} (\cite{bullet_physics_library}). The \texttt{GraspIt!} toolbox relies on Bullet, whereas \texttt{OpenRAVE} has an interface allowing the use of either ODE and Bullet.

To simulate dynamic rigid body interactions, these engines rely on constraint-based methods (\cite{baraff1993non}). In particular, for each discrete time-step of the simulation, a set of constraints is defined, reflecting properties and situation of the considered gripper, the object being grasped, and the environment. Each constraint is intended to be descriptive of the interactions between two given rigid bodies, defining reaction forces descriptive of contacts between such bodies (including impacts, support, or reflecting exchanges of efforts in joints). From the considered constraint is inferred an appropriate effort being applied on the involved objects. For instance, hinge joint constraints define reactive forces that ensure the two considered bodies are kept in contact at the hinge position; they are left free to rotate around the specified axis, but other relative movements are entirely compensated by the constraint effort. Of particular relevance to grasping are contact constraints, which prevent objects from physically overlapping. They are implemented in manner that is similar to the aforementioned hinge constraint. In particular, upon detection of the emergence of one such contact, a constraint enforcing non-overlap is added to the previously considered ones (see the discussion in \cite{baraff1993non}). The constraint prevents body movement in the direction of the contact point, preventing overlap. Different approaches may be used to infer appropriate efforts from the defined set of constraints, one of the most commonly encountered method formulates a Linear Complementary Problem (LCP \cite{cottle2009}), which may be solved using a number of different techniques (see \cite{anitescu_time_stepping_lcp_solver,lemke_lcp_solver}). Once evaluated, constraint forces are applied to concerned rigid bodies, thereby affecting their trajectory in the desired manner (see discussion in \cite{extending_ode_robots}).

Constraint-based approaches perform appropriately for a certain range of scenarii. However, a number of situations may give rise to substantial issues. For instance, rapid relative movement of objects, if simulation time steps are not carefully adjusted, may result in actual overlap between the bodies; this overlap occurring before the contact is detected and appropriate constraint forces are generated to avoid this situation. A straightforward mitigating measure to such issues consists in carefully monitoring for such abhorrences, and adjusting (that is, reducing) the simulation time-step to a degree that is commensurate with relative velocity of the concerned objects. However, such methods add considerable complexity and offer no guarantee of success (\cite{engine_simulation}). Another situation in which such overlaps commonly occur (when working in discrete time numerical simulation) is that involving closed mechanical chains. Grasping, when a gripper applies efforts on an object from different, opposing directions falls into that category. The situation is particularly prevalent when considering force-closure grasp (\cite{nguyen1988constructing}). Successfully enforcing non-overlap constraints in such situations requires particularly small simulation time steps. In the event that an overlap ends up occurring, LCP based methods typically fail, as such situations are not foreseen (\cite{baraff_analytical}).

A number of results can be found in  the literature to address such issues. A common approach involves accounting for the possibility of overlaps (which is essentially inherent to discrete-time simulation), and compute reaction forces in such a manner that, when such situation do occur, they only exist in short transient state, rapidly replaced with a steady-state situation in which contacts and interactions faithfully their real-world, physical reality. The approach in \cite{yamane2008}, for instance, defines a set of criteria to overcome inter-body penetrations. These result in the application of a repulsive force to overlapping objects, proportional to their relative velocity, at the point(s) of contact. The approach implies a number of additional steps to the simulation which may prove exceedingly computationally intensive, to the extent that real-time computations are in practice difficult to achieve. In addition, the defined repulsive forces can in some configurations lead to the emergence of a resonance effect, destabilizing force-closed grasps. Numerical simulation of grasping using such an approach typically requires the addition of artificial, large damping efforts diffusing excess energy (see \cite{engine_simulation}). Another approach involves the replacement of constraints with impulses to describe interactions, as in \cite{impulse_based}. The approach is able to account for overlap of rigid bodies. However, the reliance on impulses may lead to inaccuracies (see discussion in \cite{impulse_based}). A manner to directly address and account for overlaps consists in treating such instances not as an anomaly, but rather as an error to be reduced (or regulated). This can be pursued by defining repulsion forces in light of these errors, in a manner that concerned objects are pushed apart, as described in \cite{drumwright_penalty_based}. Penalty-based methods offer a rapid and robust method to address simulation scenarii in which objects intersect with each other, solution allowing to consider thousands of objects in real-time have been demonstrated (\cite{fast_penalty_based,drumwright_fast_penalty}). However, the penalty parameters must be selected for specific objects and collision scenarios. Should a scenario change too drastically, improperly tuned parameters could lead to oscillating behavior, as discussed in \cite{mirtich1998}. As grasping presents a situation where objects should remain in contact at specific positions, these limitations are not of consequence.
In the following, we build upon this penalty-based perspective, to develop an algorithm supporting reliable numerical simulation of robotic grasping. In particular, we ground the definition of the penalty efforts, computed from measured overlaps, in considerations of mechanical impedance (including stiffness and damping), designed to reflect the expected behavior of the considered objects in their interactions.

This paper is structured as follows. \sec{approach} provides an overview of the proposed approach, and results of illustrative numerical simulations are provided in \sec{simulations}. \sec{conclusion} concludes this paper. 

==> sections/numerical_results_grasp_and_throw.tex <==
%
\begin{figure*}
	\centering
	%\def\svgwidth{\columnwidth}
	\includegraphics[width=\textwidth]{images/grasp_throw_7.eps}
	\caption{Grasping an object and throwing it into box}
	\label{fig:grasp_throw}
\end{figure*}

Once appropriate parameters have been determined, we can simulate more complex scenarios. Here, a pick-and-throw operation is modeled. An hourglass-shaped object is placed on the floor next to a box. The gripper moves itself over the object, in a position from which it can easily grasp the object. The fingers close, locking the object in place. In contrast with other simulators that often encounter problems with this scenario, our physics simulation remains steady. This is due to the fact that our approach takes overlaps into account, and reduces knockback through the simulation of mechanical impedance, which prevents objects from bouncing around in a completed grasp.
%TODO: Explain numerical instability of other solvers better

The following describes the outcomes of individual steps in greater detail.
Once the object is grasped, the gripper lifts it up. The finger contacts transfer forces to the object, countering the simulation's gravity. Next, the object is thrown towards the box. The throw demonstrates the simulations capability of modeling impulse transfer from one object to another, in this case from the finger to the object. At launch, the previously grasped body has attained enough velocity to continue traveling away from the finger.
After following the throw's trajectory, the object lands inside the target box. Here, friction forces act upon the body, and it comes to rest once more.
The entire process is illustrated in figure \ref{fig:grasp_throw}. 

==> sections/numerical_results_wall_impact.tex <==
\subsection{Wall Impact} \label{sec:experimental_tuning}
%
A collision with a wall is a very simple scenario. We can manually compute the expected contact forces by hand and thus adjust the parametric gains $k_P$ and $k_D$ of our PD controller. Afterwards, we can use these values and see how they fare in more complex experiments.

%\begin{figure}
%	\centering
\begin{figure}%{0.45\columnwidth}
	\centering
	%\def\svgwidth{\columnwidth}
	\includegraphics[width=0.7\columnwidth]{images/wall_collision.png}
	\caption{Simple wall collision trajectory}
	\label{fig:wall_collision}
\end{figure}%
\begin{figure}%{0.45\columnwidth}
	\centering
	%\def\svgwidth{\columnwidth}
	%\includesvg[width=.9\columnwidth]{images/wall_collision_pos.svg}
	\includegraphics[width=.8\columnwidth]{images/wall_collision_pos.pdf}
	\caption{Comparison of Wall Collision trajectory between simulation and mathematically computed result}
	\label{fig:wall_collision_graph}
\end{figure}
%\end{figure}

The simulation itself comprises a rectangular object, a wall and floor (see figure \ref{fig:wall_collision}). Normal gravity of $9.81 \text{m s}^{-2}$ is acting on the object. The horizontal object starting velocity is set to $1\text{m s}^{-1}$.
To properly calibrate the $k_P$ and $k_D$ parameters, we compare the simulated trajectory with the correct trajectory that would result from a stiff collision with the wall. The latter can be trivially computed mathematically, thus being a good basis for tuning. Upon completion of the experiment, we determine that the parameters $k_P = 3967\;\text{kg}\;\text{s}^{-2}$ and $k_D = -97\;\text{kg}\;\text{s}^{-1}$
approximate the real-life trajectory rather well. Both simulated and expected trajectories are described in figures \ref{fig:wall_collision} and \ref{fig:wall_collision_graph}. The following experiments will all be using the computed parameters. 
